V2CE: Video to Continuous Events Simulator

Dynamic Vision Sensor (DVS)-based solutions have recently garnered significant interest across various computer vision tasks, offering notable benefits in terms of dynamic range, temporal resolution, and inference speed. However, as a relatively nascent vision sensor compared to Active Pixel Sensor (APS) devices such as RGB cameras, DVS suffers from a dearth of ample labeled datasets. Prior efforts to convert APS data into events often grapple with issues such as a considerable domain shift from real events, the absence of quantified validation, and layering problems within the time axis. In this paper, we present a novel method for video-to-events stream conversion from multiple perspectives, considering the specific characteristics of DVS. A series of carefully designed losses helps enhance the quality of generated event voxels significantly. We also propose a novel local dynamic-aware timestamp inference strategy to accurately recover event timestamps from event voxels in a continuous fashion and eliminate the temporal layering problem. Results from rigorous validation through quantified metrics at all stages of the pipeline establish our method unquestionably as the current state-of-the-art (SOTA).

==> contents/related_work.tex <==
% \textbf{Human Pose Estimation:} Existing methods for 3D human pose estimation can be classified into two categories: monocular \cite{Chen2020MonocularHP} and multi-view \cite{Rhodin2018LearningM3} method. The multi-view method observes subjects from multiple views/cameras from different vantage points \cite{Ge2016Robust3H}. The multi-view method requires significantly more power, and is more complex and expensive to set up, which limits its usage outside of the lab. 
% Human pose estimation methods can also be classified in another way: model-based \cite{Omran2018NeuralBF} or skeleton-based \cite{Chen2022AnatomyAware3H} methods. Model-based method attempts to reconstruct the full 3D body shape of a human model \cite{Hassan2019Resolving3H}, while skeleton-based methods use a bone skeleton as an intermediate representation, and regress the joint locations in 3D space. In this work, we use a monocular skeleton-based approach that can allow us to achieve a more efficient and practical solution for 3D human pose estimation in real-world settings.

% \textbf{Dynamic Vision Sensor(DVS)}, or event camera was originally proposed by Lichtsteiner et al. \cite{lichtsteiner2008128}. In recent years, event camera has gained increasingly more attention and has been applied to many computer vision tasks including object recognition \cite{li2021graph, kim2021n}, segmentation \cite{alonso2019ev}, gesture recognition \cite{Calabrese2019DHP19DV, Wang2019EVGaitER, Ghosh2019SpatiotemporalFF}, depth estimation \cite{gehrig2021combining, hidalgo2020learning}, Simultaneous Localization And Mapping (SLAM) \cite{jiao2021comparing, bertrand2020embedded}, and autonomous driving \cite{li2019event, chen2020event}. While RGB cameras struggle due to motion blur, event camera by design is highly sensitive to lux variation in both extremely overexposed and underexposed scene \cite{Berthelon2018EffectsOC}. In this work, we present \emph{YeLan} that leverages Event Camera for 3D human pose estimation in more realistic settings.


% Although event camera has already been adopted for human pose estimation in previous works, these works primarily focused on designing algorithms that are relatively noise-free, background-activity-less, and well-lit settings. For example, a recent event camera HPE dataset, DHP19 \cite{Calabrese2019DHP19DV} contains a series of event recordings of human movements, poses, and moving objects. Some event camera datasets are used in gesture recognition \cite{Amir2017ALP} and action recognition \cite{Hu2016DVSBD}. However, these datasets capture a limited number of motion trajectories in overly controlled environments. The lack of a diversified dataset in realistic conditions under low and dynamic light is a major bottleneck for developing a robust event camera-based sensing system. We collected a new dataset to tackle this challenge and built a comprehensive motion-to-event simulator to provide massive pre-training data to lower the cost of dataset collection.


% \textbf{High/Low Level Stream Structure Awareness} Physical att loss, GAN loss


% \textbf{temporal and noise} hierarchical temporal attention 


% \textbf{Backbone} cnn, gnn, snn

% Start from here

% Standard RGB videos have fixed and low frame rates compared to the pixel-wise event frequency of DVS camera. Consequently, prior studies \cite{Gehrig2019VideoTE}\cite{Hu2021-v2e-cvpr-workshop-eventvision2021} have proposed upsampling network to interpolate video frames between two consecutive frames. The ESIM \cite{pmlr-v87-rebecq18a, Gehrig_2020_CVPR} method is the first major work on RGB to Event translation that uses a non-ML-based adaptive sampling method. However, adaptive sampling fails to fit a long sequence of a semantically meaningful event cluster, causing ambiguity of individual events which could lead to an inconsistent sequence. The v2e method \cite{Hu2021-v2e-cvpr-workshop-eventvision2021} tries to mimic the underlying mechanism of DVS camera and employs a logarithm function on the grayscale image frames and a threshold to generate the pixel-wise DVS events. However, the resulting pixel-wise event stream from v2e fails to precisely estimate the event timings between two RGB frames. The generated event streams by the state-of-the-art v2e are cluttered or stacked around the RGB video frames. The continuous event dynamics between two adjacent RGB video frames are completely lost. Another problem with adopting a logarithm on grayscale images is that the information within the low-lighting area is completely lost. Although DVS camera has a significantly higher dynamic range than the traditional RGB camera\cite{10168206}\cite{liu2022lowlight}, we want to preserve as much information within low-lighting areas as possible to reconstruct realistic event streams.

Existing research on translating RGB videos to dynamic vision sensor (DVS) event streams\cite{Gehrig2019VideoTE}\cite{Hu2021-v2e-cvpr-workshop-eventvision2021}  is marked by several noteworthy attempts. The ESIM method \cite{pmlr-v87-rebecq18a, Gehrig_2020_CVPR}, one of the pioneering approaches in this field, utilizes a non-ML adaptive sampling technique. Nevertheless, it encounters limitations in generating a cohesive long sequence of semantically meaningful event clusters, thereby introducing potential inconsistency in the event sequence. On the other hand, the v2e method \cite{Hu2021-v2e-cvpr-workshop-eventvision2021} seeks to replicate the intrinsic mechanisms of a DVS camera. It adopts a logarithm function on grayscale image frames coupled with a threshold to generate pixel-wise DVS events. However, this approach demonstrates a significant drawback in accurately pinpointing event timings between two RGB frames, often resulting in cluttered or stacked event streams around the RGB frames and losing continuity in event dynamics between adjacent frames. Furthermore, given the higher dynamic range of DVS cameras compared to traditional RGB cameras \cite{10168206, liu2022lowlight}, this approach tends to overlook information in low-light areas which is a gap that stands contrary to the objective of retaining as much data as possible in such regions to fabricate realistic event streams. In summation, while existing methods mark a significant stride towards RGB to DVS translation, they present shortcomings in accurately preserving event dynamics and information richness, especially in low-light conditions. Future research should aspire to mitigate these challenges, paving the way for more realistic and consistent event stream translations.



% The EventGAN method \cite{zhu2019eventgan} utilizes generative adversarial network\cite{goodfellow2014generative} to generate a continuous event stream. The generated events are sent to two independent Event-to-Flow~\cite{ParedesValls2018UnsupervisedLO, gehrig2021eraft} network and Event-to-Image~\cite{9191114, Duwek2021ImageRF} network which attempt to reconstruct original RGB information from generated events. However, the EventGAN method relies heavily on the performance of the Event-to-Flow model and the Event-to-Image model which increases the overall system's complexity. While the integration of multiple pipelines might be intended to augment the robustness of the predictions, it inadvertently creates a fragile foundation where the underperformance or malfunction of the Event-to-Flow or the Event-to-Image model can precipitate a cascade of failures or inaccuracies throughout the pipeline. Another problem is that EventGAN only predicts event streams between two consecutive frames since the temporal context is relatively short between two contiguous frames. Given the intrinsic high-frequency property of DVS camera which our work is focusing on, the short temporal context of EventGAN could result in inconsistent semantics within a consecutive long image sequence. Considering the sparsity of event streams, the Graph Neural Networks (GNN)~\cite{Scarselli2009TheGN} and Spiking Neural Networks (SNN)~\cite{Tavanaei2018DeepLI, Deng2022TemporalET} are natural fit and can offer more energy-efficient and fast processing of the DVS data~\cite{10166491,schaefer2022aegnn,cordone2021learning,zhu2022eventbased} without needing any frame-based data accumulation. In the context of GNN, edge connections are heavily reliant on the local microstructure. Clustering events around RGB video frame or inaccurate event timing estimation (discussed above) alters the edge connections pattern causing a domain shift. SNN also suffers from the same problem since the causal relationship between two successive event firings can not be harnessed due to the intrinsic inaccurate event timings. In this work, we aim to harness the higher-order dynamics of an object's motion and pixel-wise intensity changes to accurately estimate the total number of events between two RGB video frames and more importantly accurately estimate the event timing to generate a more realistic event stream from video data.

The EventGAN method \cite{zhu2019eventgan} employs a generative adversarial network (GAN) \cite{goodfellow2014generative} to create a continuous event stream, which is then fed into separate Event-to-Flow \cite{ParedesValls2018UnsupervisedLO, gehrig2021eraft} and Event-to-Image \cite{9191114, Duwek2021ImageRF} networks to reconstruct the original RGB data. However, this approach is fraught with challenges, particularly the high dependency on the performance of the secondary networks, which raises the system complexity and creates potential weak links that can propagate errors throughout the pipeline. Additionally, EventGAN is restricted by a short temporal context, generating event streams only between two successive frames. It is a limitation that can cause inconsistency in semantic representation over longer sequences. Given the high-frequency characteristics of DVS cameras, which are the focus of our study, alternative approaches such as Graph Neural Networks (GNN) \cite{Scarselli2009TheGN} and Spiking Neural Networks (SNN) \cite{Tavanaei2018DeepLI, Deng2022TemporalET} are naturally aligned to offer energy-efficient and swift processing of DVS data \cite{10166491,schaefer2022aegnn,cordone2021learning,zhu2022eventbased} without the necessity for frame-based data accumulation. However, they too grapple with challenges: the GNN’s dependency on local microstructure makes them vulnerable to alterations in edge connection patterns, and similarly, the SNN struggles to leverage the causal relationships between successive event firings due to the inherent inaccuracies in event timings. In our research, we seek to bridge these gaps by focusing on the meticulous estimation of event timings and discerning higher-order dynamics such as object motion and pixel-wise intensity variations. Our objective is to accurately gauge the volume of events between two RGB video frames and hone the estimation of event timings, fostering a more authentic translation from video data to event streams.

% occurring at the same pixel but at different timestamps may indicate a causal relationship during training. However, when these generated events are assigned the same timestamp, this correlation could be altered, which could lead to complications when these synthesized data are utilized for pretraining.


